Generating API Parameter Security Rules with LLM for API Misuse Detection

In this paper, we present a new framework, named GPTAid, for automatic APSRs generation by analyzing API source code with LLM and detecting API misuse caused by incorrect parameter use. To validate the correctness of the LLM-generated APSRs, we propose an execution feedback-checking approach based on the observation that security-critical API misuse is often caused by APSRs violations, and most of them result in runtime errors. Specifically, GPTAid first uses LLM to generate raw APSRs and the Right calling code, and then generates Violation code for each raw APSR by modifying the Right calling code using LLM. Subsequently, GPTAid performs dynamic execution on each piece of Violation code and further filters out the incorrect APSRs based on runtime errors. To further generate concrete APSRs, GPTAid employs a code differential analysis to refine the filtered ones. Particularly, as the programming language is more precise than natural language, GPTAid identifies the key operations within Violation code by differential analysis, and then generates the corresponding concrete APSR based on the aforementioned operations. These concrete APSRs could be precisely interpreted into applicable detection code, which proven to be effective in API misuse detection. Implementing on the dataset containing 200 randomly selected APIs from eight popular libraries, GPTAid achieves a precision of 92.3%. Moreover, it generates 6 times more APSRs than state-of-the-art detectors on a comparison dataset of previously reported bugs and APSRs. We further evaluated GPTAid on 47 applications, 210 unknown security bugs were found potentially resulting in severe security issues (e.g., system crashes), 150 of which have been confirmed by developers after our reports.

==> Sections/prompt-listing.tex <==
\begin{lstlisting}[frame=trBL,caption= {Prompt template for Raw PRSRs Generation},abovecaptionskip=10pt,belowcaptionskip=0pt,captionpos=b,label={lst:prompt-rule}, 
basicstyle=\footnotesize\ttfamily,
breaklines=true, float=!h
]
source code of `FUNC_NAME`:
```
SOURCE_CODE
```

Please analyze the source code of the API `FUNC_NAME` and all the information provided before it. Then, respond with the following tasks:

Task 1: Based on the analysis of the source code, provide a concise description of the functionality of the function.

Task 2: Locate the code related to the Parameter_Info `PARA_NAME`.

Task 3: Identify the security rules that should be observed for the Parameter_Info to prevent misuse of the API `FUNC_NAME`. For each rule, include code snippets that demonstrate a violation of the rule:

    1. Please provide detailed and specific descriptions for each rule. Clearly indicate which specific operations relate to the Parameter_Info. If a rule can apply to multiple operations that breach the rule, please make it more specific.
    
    2. Each rule should focus on describing only one behavior if possible. If a rule encompasses multiple behaviors, please break it down into distinct rules.
    
    3. Each rule should correspond to a separate violation code.
    
    4. In cases where you're unsure about certain code details, you can suggest all possible rules, whether accurate or not, based on your knowledge database about potential API misuse.
    
    5. Each violation code should contain at least one call to `FUNC_NAME`
    
    6. Follow this format for each rule: Begin with an Arabic numeral, then describe the rule content (e.g., "1. Rule description"). Provide a corresponding violation code enclosed in triple backticks like this:
    ```
    //Violation Code
    ```
    Format Example For Each Rule:
    (Note: These examples are provided only for reference and should not influence the format of the responses.)
    1. Rule:
    Violation Code:
    ```
    //Violation Code
    ```
    1. Rule:
    Violation Code:
    ```
    //Violation Code
    ```
\end{lstlisting}

\begin{lstlisting}[frame=trBL,caption= {Prompt template for Right Code Generation},abovecaptionskip=10pt,belowcaptionskip=0pt,captionpos=b,label={lst:prompt-right}, 
basicstyle=\footnotesize\ttfamily,
breaklines=true, float=!t
]
Given the following function `FUNC_NAME` in library `LIB_NAME`, Complete the following tasks.
Task1: Analyze the function code to find the invocation specification that the caller needs to follow correctly.
Task2: Generate a complete code that calls the function in Linux. The code needs to meet the following requirements:
    1.The code is required to be compilable and follow the invocation specification of this function.
    2.This code needs to be non-interactive and no infinite loops.
    3.The code needs to check the call status of each API after the API returns(if API status can be checked). If API call fails, return 123 and output error message to infer the cause of the error. Every `printf` need to be different.
    4. After any `printf`, please flush the stdout. 
    5. Output: "Calling FUNC_NAME success" after calling `FUNC_NAME` successfully; Output: "Calling FUNC_NAME fail" after the call to `FUNC_NAME` has failed
    6. Add line: 
    ```
    printf("before FUNC_NAME\n")
    ```
    before calling `FUNC_NAME`. Make sure that there are no other function calls between this output and the calling to `FUNC_NAME`
    7. If there are some file read operations in the code, the file name should be `example.xxx`
    8. Be sure to output the code in this format: ```code``` 

\end{lstlisting}



\begin{lstlisting}[frame=trBL,caption= {Prompt template for Violation Code Generation},abovecaptionskip=10pt,belowcaptionskip=0pt,captionpos=b,label={lst:prompt-wrong}, 
basicstyle=\footnotesize\ttfamily,
breaklines=true, float=!t
]
Info: 
"""
1.Declaration of `FUNC_NAME`:
```
DECLARATION_REPLACE
```
2.Right Code that calls `FUNC_NAME`:
```
RIGHT_CODE_REPLACE
```
"""
Based on the above information, please modify the right code to violate this rule:
RULE_NAME
Here is an example of a code that violates the rule; analyze the code to determine how to violate the rule by modifying the right code, as this violation example code indicates. Your modified code must to be consistent with the way the example code is violated.
violation code example:
```
VIOLATION
```
\end{lstlisting}

\begin{lstlisting}[frame=trBL,caption= {Prompt template for PRSRs Refinement (one wrong code in a group)},abovecaptionskip=10pt,belowcaptionskip=0pt,captionpos=b,label={lst:prompt-refine_one}, 
basicstyle=\footnotesize\ttfamily,
breaklines=true
]
Given the information provided, please perform a likelihood-based analysis to determine the most probable causes of the error. Subsequently, generate security rules that address these causes. Understand that both the correct and incorrect API calls might have multiple modifications, so consider a range of possibilities and rank them based on their likelihood.
Target API is: `FUNC_NAME`
Info 0. Declaration of FUNC_NAME:
DECLARATION

Info 1. Correct API Call:
```
RIGHT_CODE
```

Info 2. Error Code resulting from a potential security rule violation:
```
VIOLATION
```

Info 3. Error Results of the Run when the rule might be violated:
ERROR_RE

Info 4. Rule that might related to this situation:
RULE_NAME

Steps for Analysis:

1. Enumerate the key differences between the correct(Info 1) and error(Info 2) API calls.
2. Analyze the possible status of this parameter in the correct code(Info 1).
If you can determine the possible value of the parameter, then the status is represented by that value, and if you can't determine the possible value, then the status is represented by the operation associated with the parameter (function call sequence)
3. Analyze the possible status of this parameter in the error code(Info 2).
Same definition of possible status as the previous step.
4. Determine the potential root cause of the error based on the error results(Info 3).
5. Check if the rule(Info 4) above is related to this error.
6. For each identified difference, evaluate its probability of being the primary root cause of the error based on the provided error code and Result of the Run.
7. Rank these causes based on their likelihood.
8. Analyse which parameter related to the root cause. Answer the index of the parameter, index begin with 1.
9. For the most probable causes, gesnerate specific security rules to prevent such errors in the future.
Generate a single parameter-related rule that includes the index(begin with 1) and name of the parameter causing the error, along with specific actions or value to address the ROOT CAUSE effectively.
The Rule you generate should contain 3 part infomation: 
    (1)index and name of the parameter
    (2)What the caller of this API must do to avoid this error
    (3)What the caller of this API must not do to avoid this error.
Do not include any information or associations with other error cases in the generated rule.

Please provide the rule in the following format so I can parse your response automatically:
    A. Security Rule AUTO: Parameter [INDEX](begin with 1): [what the caller MUST DO]
    B. Security Rule AUTO_AVOID: Parameter [INDEX](begin with 1): [what the caller MUST NOT DO]
    you should replace the content enclosed in square brackets "[ ]" with your answer.
Explaination: 
Show me your analyze step following above steps
\end{lstlisting}

\begin{lstlisting}[frame=trBL,caption= {Prompt template for PRSRs Refinement(multi-wrong code in a group)},abovecaptionskip=10pt,belowcaptionskip=0pt,captionpos=b,label={lst:prompt-refine_multi}, 
basicstyle=\footnotesize\ttfamily,
breaklines=true, float=!h
]
Given the information provided, please perform a likelihood-based analysis to determine the most probable causes of the error. Subsequently, generate security rules that address these causes. Understand that both the correct and incorrect API calls might have multiple modifications, so consider a range of possibilities and rank them based on their likelihood.
Target API is: `FUNC_NAME`
Info 0. Declaration of FUNC_NAME:
DECLARATION

Info 1. Correct API Call:
```
RIGHT_CODE
```

Info 2. Error Code resulting from a potential security rule violation:
```
VIOLATION
```

Info 3. Error Results of the Run when the rule might be violated:
ERROR_RE

Steps for Analysis:

1. Enumerate the key differences between the correct(Info 1) and error(Info 2) API calls.
2. Analyze the possible status of the parameter in the correct code(Info 1).
If you can determine the possible value of the parameter, then the status is represented by that value, and if you can't determine the possible value, then the status is represented by the operation associated with the parameter (function call sequence)
3. Analyze the possible status of the parameter in the error code(Info 2).
Same definition of possible status as the previous step.
4. Determine the potential root cause of the error based on the error results(Info 3).
5. For each identified difference, evaluate its probability of being the primary root cause of the error based on the provided error code and Result of the Run.
6. Rank these causes based on their likelihood.
7. Analyse which parameter related to the root cause. Answer the index of the parameter, index begin with 1.
8. For the most probable causes, gesnerate specific security rules to prevent such errors in the future.
Generate a single parameter-related rule that includes the index(begin with 1) and name of the parameter causing the error, along with specific actions or value to address the ROOT CAUSE effectively.
The Rule you generate should contain 3 part infomation: 
    (1)index and name of the parameter
    (2)What the caller of this API must do to avoid this error
    (3)What the caller of this API must not do to avoid this error.
Do not include any information or associations with other error cases in the generated rule.

Please provide the rule in the following format so I can parse your response automatically:
    A. Security Rule AUTO: "Parameter [INDEX](begin with 1): [what the caller MUST DO]
    B. Security Rule AUTO_AVOID: "Parameter [INDEX](begin with 1): [what the caller MUST NOT DO]
    you should replace the content enclosed in square brackets "[ ]" with your answer.
Explaination: 
Show me your analyze step following above steps

\end{lstlisting}

==> Sections/prompt.tex <==


\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{Figure/cprompt-right.pdf}
    \caption{Prompt template for Right Code Generation} 
\label{fig:cprompt-right}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{Figure/cprompt-violation.pdf}
    \caption{Prompt template for Violation Code Generation} 
\label{fig:cprompt-violation}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{Figure/cprompt-refine-one.pdf}
    \caption{Prompt template for PRSRs Refinement (one violation code in a group)} 
\label{fig:cprompt-refine-one}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{Figure/cprompt-refine-multi.pdf}
    \caption{Prompt template for PRSRs Refinement (multiple violation code in a group)} 
\label{fig:cprompt-refine=multi}
\end{figure}



==> Sections/todo_list.tex <==
JH:
1.
2. top 20-30 lib
    Context: API -> original/human name/fruit name
    Question1: What/Who does allocate/free? What/Who perform allocating/freeing?  What/Who allocates/frees? 

    Who does allocation/free

    TP=XXX FP TN TP
    precis... recall

12.31
@JH

FP: 人标记的为0，模型预测出来时1 | QA错标了1 -> 人 operator = 0, QA：XXX | operator = API name ,1 (XXX)，QA: API2, YYY -> FP++
FN: 人标记的为1，模型预测出来是0 -> 人operator = API name, 1（XXX）,QA：没有（< confidence）-> FN ++
TP: 人标记的为1，模型预测出来也是1 -> 人operator = API name, 1（XXX）, QA：API name，XXX -> TP++
TN: 人标记的为0，模型预测出来也是0 -> 人 operator = 0，QA：没有（< confidence）-> TN++

precision = TP/(TP+FP)
recall = TP/(TP+FN)

-----

Question:
keywords
allocate allocating allocation
create creating creation
initialize initializing initialization
construct constucting construction
deallocate deallocating deallocation
free free 
release releasing release

What allocates?
What dose allocating? X
What dose the allocation? X
What do allocate? X
What do allocating? X
What do the allocation? X
What did allocating? X
What did the allocation? X
What performs allocating?
What performs the allocating?
What is allocating? X
Who allocates?
Who dose allocating?
Who dose the allocation?
Who do allocate?
Who do allocating?
Who do the allocation?
Who did allocating?
Who did the allocation?
Who performs allocating?
Who performs the allocating?
Who is allocating?

------------


